Critical Ising model, Multiple SLE$_\kappa\left(\frac{\kappa-6}{2},\frac{\kappa-6}{2}\right)$ and $\beta$-Jacobi Ensemble

Fix $N\ge 1$ and suppose that $(\Omega;x_1,\ldots, x_{N}; x_{N+1}, x_{N+2})$ is a polygon, i.e. $\Omega$ is a simply connected domain with locally connected boundary and $x_1,\ldots,x_{N+2}$ are $N+2$ different points located counterclockwisely on $\partial\Omega$. Fix $\kappa\in (0,4)$. In this paper, we will give two different constructions of multiple $N$-SLE$_\kappa\left(\frac{\kappa-6}{2},\frac{\kappa-6}{2}\right)$ on $(\Omega;x_1,\ldots,x_{N}; x_{N+1},x_{N+2})$ and prove that they give the same law on random curves. Then, by establishing the uniqueness of multiple $N$-SLE$_\kappa\left(\frac{\kappa-6}{2},\frac{\kappa-6}{2}\right)$, we can obtain the joint law of the hitting points of multiple $N$-SLE$_\kappa\left(\frac{\kappa-6}{2},\frac{\kappa-6}{2}\right)$ with odd (resp. even) indices on $(x_{N+1}x_{N+2})$. After shrinking $x_1,\ldots,x_N$ to one point, the law of hitting points with odd (resp. even) indices converge to $\beta$-Jacobi ensemble with the conjectured relation $\beta=\frac{8}{\kappa}$. We will establish a direct connection between SLE-type curves and $\beta$-Jacobi ensemble. As an application, we consider critical Ising model on a discrete polygon $(\Omega^\delta_\delta;x^\delta_1,\ldots,x^\delta_{N}; x^\delta_{N+1},x^\delta_{N+2})$ with alternating boundary $(x^\delta_{N+2}x^\delta_{N+1})$ and free boundary $(x^\delta_{N+1}x^\delta_{N+2})$. Motivated by the partition function of multiple $N$-SLE$_\kappa\left(\frac{\kappa-6}{2},\frac{\kappa-6}{2}\right)$, we derive the scaling limit of the probability of the event that the interface $\gamma_j^\delta$ starting from $x^\delta_j$ ends at $(x^\delta_{N+1}x^\delta_{N+2})$ for all $1\le j\le N$. Moreover, we prove that given this event, the interface $(\gamma_1^\delta,\ldots,\gamma_N^\delta)$ converges to multiple $N$-SLE$_\kappa\left(\frac{\kappa-6}{2},\frac{\kappa-6}{2}\right)$ with $\kappa=3$.

==> Ising.tex <==
In this section, we will prove Theorem~\ref{thm::Ising_limit}.  Recall that we denote by $\gamma_j^\delta$ the interface starting from $x_j^\delta$ for $1\le j\le N$. We first recall the convergence of the law of $\gamma_j^\delta$ as $\delta\to 0$.
\begin{lemma}\label{lem::conv_aux}
Use the same notations as in Theorem~\ref{thm::Ising_limit}. For $1\le j\le N$, the law of $\gamma_j^\delta$ converges as $\delta\to 0$. Denote by $\gamma_j$ the limit. Denote by $(W_t^{\gamma_j}:t\ge 0)$ the driving function of $\phi(\gamma_j)$ and by $(g_t^{\gamma_j}:t\ge 0)$ the corresponding conformal map. Denote by $T$ the hitting time of $\gamma_j$ at the union of $\{x_1,\ldots,x_{j-1},x_{j+1},\ldots,x_{N},x_{N+1},x_{N+2}\}$ and the free boundary $(x_{N+1}x_{N+2})$. Then, before time $T$, the driving function $W^{\gamma_j}$ satisfies the SDE
\begin{equation}\label{eqn::local_driving}
\ud W_t^{\gamma_j}=\sqrt 3\ud B_t+\partial_j \log R(g^{\gamma_j}_t(\phi(x_1)),\ldots,g^{\gamma_j}_t(\phi(x_{j-1})), W_t^{\gamma_j}, g^{\gamma_j}_t(\phi(x_{j+1})), \ldots,g^{\gamma_j}_t(\phi(x_N));g^{\gamma_j}_t(\phi(x_{N+1})))\ud t,
\end{equation}
where $B$ is the standard Brownian motion.
\end{lemma}
\begin{proof}
The conclusion is the combination of Lemma 3.4 and Lemma 3.6 in~\cite{FengWuYangIsing} after mapping from $\mathbb D$ to $\HH$. Below, we explain it briefly.
\begin{itemize}
\item
The convergence of the driving function has been proved in~\cite[Theorem 3.1]{IzyurovObservableFree}. Note that in~\cite[Theorem 3.1]{IzyurovObservableFree}, we only need the convergence of $\{(\Omega_\delta;x_1^\delta,\ldots,x_N^\delta;x_{N+1}^\delta,x_{N+2}^\delta)\}_{\delta>0}$ to $(\Omega;x_1,\ldots,x_N;x_{N+1},x_{N+2})$ in the Carath\'eodory sense.
\item
The proof of $\gamma_j^\delta$ under the metric~\ref{eqn::curve_metric} is similar to the proof of~\cite[Theorem 5.1 and Proposition 6.1]{KarrilaMultipleSLELocalGlobal}.
\end{itemize}
This completes the proof.
\end{proof}
Note that in Lemma~\ref{lem::conv_aux}, we do not prove that $\gamma_j$ hits $\partial\Omega$ only at its two ends for $1\le j\le N$, which is crucial in the proof of Theorem~\ref{thm::Ising_limit}. In Lemma~\ref{lem::conv_aux1}, we will give a uniform control of such events in discrete setting for $\delta>0$.
\begin{lemma}\label{lem::conv_aux1}
Fix $1\le j\le N$. For every $\eps>0$ and $\delta>0$, denote by $\sigma_{j,\eps}^\delta$ (resp. $\tau_{j,\eps}^\delta$) the hitting time of $\gamma_j^\delta$ at the $\eps$-neighbourhood of $\{x_1^\delta,\ldots, x_{j-1}^\delta,x_{j+1}^\delta,\ldots,x_N^\delta\}$ (resp. $(x_{N+1}^\delta x_{N+2}^\delta)$). Then, there exists constants $C_1>0$ and $C_2>0$, such that
\begin{equation}\label{eqn::error_estimate1}
\PP[\sigma_{j,\eps}^\delta<\infty, \text{ and }\gamma_j^\delta\text{ ends at }(x_{N+1}^\delta x_{N+2}^\delta)]\le C_1\eps^{C_2}.
\end{equation}
and
\begin{equation}\label{eqn::error_estimate2}
\PP[\tau_{j,\eps}^\delta<\infty,\text{ and then }\gamma_j^\delta\text{ hits }\partial B(\gamma_j^\delta(\tau_{j,\eps}^\delta),\sqrt\eps)\text{ before hitting }(x_{N+1}^\delta x_{N+2}^\delta)] \le C_1\eps^{C_2}
\end{equation}
and
\begin{equation}\label{eqn::error_estimate3}
\PP\left[\gamma_j^\delta\text{ hits }\partial B(x_{N+1}^\delta,\eps)\cup \partial B(x_{N+2}^\delta,\eps)\right] \le C_1\eps^{C_2}
\end{equation}
\end{lemma}
\begin{proof}
The proof is based on the standard argument using Lemma~\ref{lem::RSW}. For completeness, we provide a proof of~\eqref{eqn::error_estimate1} when $j=N$. The other cases and~\eqref{eqn::error_estimate2} and~\eqref{eqn::error_estimate3} can be proved similarly.
We may assume that $N$ is even such that the spins on the left of $\gamma_N^\delta$ equal $+1$ and the spins on the right of  $\gamma_N^\delta$ equal $-1$.

On the event $\{\gamma_j^\delta\text{ ends at }(x_{N+1}^\delta x_{N+2}^\delta)\}$, there is a $+1$ cluster connecting $(x_{N-1}^\delta x_N^\delta)$ to $(x_{N+1}^\delta x_{N+2}^\delta)$. Denote by $\LC_N^\delta$ the leftmost one (the precise choice is not important). For $0\le\ell\le -\log_2\sqrt\eps$, we define the following domains.
\begin{itemize}
\item
Denote by $C^\delta_{\ell,k}$ the connected component of $(B(x_j^\delta, 2^\ell\eps)\setminus B(x_j^\delta, 2^{\ell-1}\eps))\setminus \LC_N^\delta$ which contains parts of $\LC_N^\delta$ on its boundary, for $1\le k\le k_\ell$. Denote by $\alpha_{\ell,k}^\delta$ and $\beta_{\ell,k}^\delta$ two crossings of $\LC_N^\delta$ on the boundary of $C^\delta_{\ell,k}$. 
Denote by $\xi_{\ell,k}$ the boundary condition such that it equals $+1$ along $\alpha_{\ell,k}^\delta$ and $\beta_{\ell,k}^\delta$, and it equals $-1$ along $\partial C^\delta_{\ell,k}\setminus (\alpha_{\ell,k}^\delta\cup\beta_{\ell,k}^\delta)$.
\item
Denote by $\alpha_\ell^\delta$ the first crossing of $\LC_N^\delta$ through $B(x_j^\delta, 2^\ell\eps)\setminus B(x_j^\delta, 2^{\ell-1}\eps)$ and by $\beta_\ell^\delta$ the last crossing. Denote by $C_\ell^\delta$ the connected component of $(B(x_j^\delta, 2^\ell\eps)\setminus B(x_j^\delta, 2^{\ell-1}\eps))\setminus \LC_N^\delta$ which contains $\alpha_\ell^\delta$ and $\beta_\ell^\delta$ on its boundary and contains $C^\delta_{\ell,k}$ for $1\le k\le k_\ell$. Denote by $\xi_{\ell}$ the boundary condition such that it equals $+1$ along $\alpha_{\ell}^\delta$ and $\beta_{\ell}^\delta$, and it equals $-1$ along $\partial C^\delta_{\ell}\setminus (\alpha_{\ell}^\delta\cup\beta_{\ell}^\delta)$.
\end{itemize}
Note that
\begin{align}\label{eqn::RSW_aux1}
&\{\sigma_{j,\eps}^\delta<\infty, \text{ and }\gamma_j^\delta\text{ ends at }(x_{N+1}^\delta x_{N+2}^\delta)\}\notag\\
\subset& \cap_{0\le\ell\le -\frac{1}{2}\log_2\sqrt\eps}\left(\cap_{1\le k\le k_\ell}\{\text{there exists }+1 \text{ crossing between }\alpha_{2\ell,k}^\delta\text{ and }\beta_{2\ell,k}^\delta\text{ on }C^\delta_{2\ell,k}\}\right)^c.
\end{align}
By domain Markov property and monotonicity, we have that
\begin{align}\label{eqn::RSW_aux2}
&\PP[\cap_{0\le\ell\le -\frac{1}{2}\log_2\sqrt\eps}\left(\cap_{1\le k\le k_\ell}\{\text{there exists }+1 \text{ crossing between }\alpha_{2\ell,k}^\delta\text{ and }\beta_{2\ell,k}^\delta\text{ on }C^\delta_{2\ell,k}\}\right)^c]\notag\\
=&\PP\left[\prod_{0\le\ell\le -\frac{1}{2}\log_2\sqrt\eps}\left(1-\prod_{1\le k\le k_\ell}\PP^{\sigma |_{\partial C^\delta_{\ell,k}}}_{C^\delta_{\ell,k}}\left[\text{there exists }+1 \text{ crossing between }\alpha_{2\ell,k}^\delta\text{ and }\beta_{2\ell,k}^\delta\text{ on }C^\delta_{2\ell,k}\right]\right)\right]\notag\\
\le &\PP\left[\prod_{0\le\ell\le -\frac{1}{2}\log_2\sqrt\eps}\left(1-\prod_{1\le k\le k_\ell}\PP^{\xi_{\ell,k}}_{C^\delta_{\ell,k}}\left[\text{there exists }+1 \text{ crossing between }\alpha_{2\ell,k}^\delta\text{ and }\beta_{2\ell,k}^\delta\text{ on }C^\delta_{2\ell,k}\right]\right)\right].
\end{align}
Still by domain Markov property and monotonicity, we have that
\begin{align}\label{eqn::RSW_aux3}
&\prod_{1\le k\le k_\ell}\PP^{\xi_{\ell,k}}_{C^\delta_{\ell,k}}\left[\text{there exists }+1 \text{ crossing between }\alpha_{2\ell,k}^\delta\text{ and }\beta_{2\ell,k}^\delta\text{ on }C^\delta_{2\ell,k}\right]\notag\\
\ge& \PP^{\xi_{\ell}}_{C^\delta_{\ell}}\left[\text{there exists }+1 \text{ crossing between }\alpha_{2\ell}^\delta\text{ and }\beta_{2\ell}^\delta\text{ on }C^\delta_{2\ell}\right]
\end{align}
Combining~\eqref{eqn::RSW_aux1}--\eqref{eqn::RSW_aux3} and Lemma~\ref{lem::RSW} together, we obtain~\eqref{eqn::error_estimate1}. This completes the proof.
\end{proof}
%\begin{lemma}\label{lem::prob_control}
%There exists a constant $c=c(\Omega;x_1,\ldots,x_{N};x_{N+1},x_{N+2})>0$, such that for every $\delta>0$, we have
%\begin{equation}\label{eqn::uniform_control}
%\PP[A_\delta]>c.
%\end{equation} 
%In particular, denote by $\PP^*_\delta$ the conditional law of $(\gamma_1^\delta,\ldots,\gamma_N^\delta)$ given $A_\delta$, we have that $\{\PP^*_\delta\}_{\delta>0}$ is tight.
%\end{lemma}
%\begin{proof}
%By Lemma~\ref{lem::conv_aux}, we obtain the tightness of $\{(\gamma_1^\delta,\ldots,\gamma_N^\delta)\}_{\delta>0}$. Combining with~\eqref{eqn::uniform_control}, we complete the proof.
%\end{proof}
By Lemma~\ref{lem::conv_aux}, we can also obtain the tightness of $\{(\gamma_1^\delta,\ldots,\gamma_N^\delta)\}_{\delta>0}$. Suppose $(\gamma_1,\ldots,\gamma_N)$ is a subsequential limit and suppose $(\gamma_1^{\delta_n},\ldots,\gamma_N^{\delta_n})$ converges to $(\gamma_1,\ldots,\gamma_N)$ in law as $n\to\infty$. By Skorokhod’s representation theorem, we can construct a coupling $\mathcal Q$ of $\{(\gamma_1^{\delta_n},\ldots,\gamma_N^{\delta_n})\}_{n\ge 1}$ and $(\gamma_1,\ldots,\gamma_N)$ such that $\gamma_j^{\delta_n}$ converges to $\gamma_j$ almost surely as $n\to\infty$. 
\begin{lemma}\label{lem::conv_aux2}
Denote by $\sigma$ (resp. $\tau$) the hitting time of $\gamma_N$ at $\{x_1,\ldots, x_{N-1}\}$ (resp. $(x_{N+1}x_{N+2})$). Under $\mathcal Q$, we have that $\one_{\{\gamma_N^{\delta_n}\text{ ends at }(x_{N+1}^\delta x_{N+2}^\delta)\}}$ converges to $\one_{\{\tau<\sigma\}}$ in probability.  Moreover, we have that $\gamma_j$ hits $\partial\Omega$ only at its two ends for $1\le j\le N$ and $\gamma_j$ does not hit $\{x_{N+1},x_{N+2}\}$.
%In particular, we have that $\one_{\{\gamma_N^{\delta_n}\text{ ends at }(x_{N+1}^\delta,x_{N+2}^\delta)\}}\gamma_N^{\delta_n}$ converges to $\one_{\{\tau<\sigma\}}\gamma_N[0,\tau]$ in law.
\end{lemma}
\begin{proof}
We will use the same notations as in Lemma~\ref{lem::conv_aux1}. Choose $\eps$ small enough. We have the following relations
\begin{align*}
&\{d(\gamma_N^{\delta_n},\gamma_N)\le\eps\}\cap\left(\{\gamma_N^{\delta_n}\text{ ends at }(x_{N+1}^\delta x_{N+2}^{\delta_n})\}\setminus\{\tau<\sigma\}\right)\\
\subset&\{\sigma_{j,\eps}^{\delta_n}<\infty, \text{ and }\gamma_j^{\delta_n}\text{ ends at }(x_{N+1}^{\delta_n}x_{N+2}^{\delta_n})\}\cup\{\gamma_N^{\delta_n}\text{ hits }\partial B(x_{N+1}^\delta,\eps)\cup \partial B(x_{N+1}^\delta,\eps)\}
\end{align*}
and
\begin{align*}
&\{d(\gamma_N^{\delta_n},\gamma_N)\le\eps\}\cap\left(\{\tau<\sigma\}\setminus(\{\gamma_N^{\delta_n}\text{ ends at }(x_{N+1}^{\delta_n}x_{N+2}^{\delta_n})\}\right)\\
\subset &\{\tau_{N,\eps}^{\delta_n}<\infty,\text{ and then }\gamma_N^{\delta_n}\text{ hits }\partial B(\gamma_N^{\delta_n}(\tau_{N,\eps}^{\delta_n}),\sqrt\eps)\text{ before hitting }(x_{N+1}^{\delta_n}x_{N+2}^{\delta_n})\}
\\
&\cup\{\gamma_N^{\delta_n}\text{ hits }\partial B(x_{N+1}^\delta,\eps)\cup \partial B(x_{N+1}^\delta,\eps)\}.
\end{align*}
Combining with Lemma~\ref{lem::conv_aux1}, we have that 
\begin{equation}\label{eqn::diff_aux}
\mathcal Q\left[\one_{\{d(\gamma_N^{\delta_n},\gamma_N)\le\eps\}}\left|\one_{\{\gamma_N^{\delta_n}\text{ ends at }(x_{N+1}^\delta x_{N+2}^{\delta_n})\}}-\one_{\{\tau<\sigma\}}\right|\right]\le C_1\eps^{C_2}.
\end{equation}
By choosing $n$ large enough, we have that
\begin{equation}\label{eqn::dis_aux}
\mathcal Q[d(\gamma_N^{\delta_n},\gamma_N)\ge\eps]<\eps.
\end{equation}
Combining~\eqref{eqn::diff_aux} and~\eqref{eqn::dis_aux} together, we have that $\one_{\{\gamma_N^{\delta_n}\text{ ends at }(x_{N+1}^\delta x_{N+2}^\delta)\}}$ converges to $\one_{\{\tau<\sigma\}}$ in probability.  By almost the same argument, we can prove that $\gamma_j$ hits $\partial\Omega$ only at its two ends for $1\le j\le N$. This completes the proof.
\end{proof}
Before the proof of Theorem~\ref{thm::Ising_limit}, we derive some useful properties of functions $\LR_N$ and $\mathcal Z_N$.
\begin{lemma}\label{lem::mart_gammaN}
FIx $N\ge 1$. The function $\LR_N$ satisfies the PDE systems: for $1\le i\le N$, we have that ($\kappa=3$ and $h=\frac{1}{2}$)
\begin{equation}\label{eqn::BPZ}
\left(\frac{\kappa}{2}\partial_{ii}^2+\sum_{\substack{1\le j\le N+1\\j\neq i}}\frac{2}{y_j-y_i}\partial_j-\sum_{\substack{1\le j\le N\\j\neq i}}\frac{2h}{(y_j-y_i)^2}-\frac{1}{8}\frac{1}{(y_{N+1}-y_i)^2}\right)R=0
\end{equation}
Moreover, let $y_j:=\phi(x_j)$ in Lemma~\ref{lem::conv_aux} for $1\le j\le N$. Suppose $\ell$ is $\SLE_\kappa\left(2,\ldots,2;\frac{\kappa-6}{2}\right)$  from $y_N$ to $\infty$ with force points $x_1^L=y_{N-1},\ldots,x_{N-1}^L=y_1$ on its left and $x_1^R=y_{N+1}$ on its right. Denote by $(W^{\ell}_t:t\ge 0)$ the driving function of $\ell$ and by $(g_t^\ell:T\ge 0)$ the corresponding conformal maps. Define 
\begin{align*}
M_t:=&\frac{\prod_{1\le i<j\le N-1}(g_t^\ell(y_j)-g_t^\ell(y_i))^{-\frac{2}{3}}\prod_{1\le i\le N-1}(g_t^\ell(y_{N+1})-g_t^\ell(y_i))^{\frac{1}{2}}}{\prod_{1\le i<j\le N-1}(y_j-y_i)^{-\frac{2}{3}}\prod_{1\le i\le N-1}(y_{N+1}-y_i)^{\frac{1}{2}}}\\
&\times \frac{(g_t^\ell(y_{N+1})-W_t^\ell)^{\frac{1}{2}}\times\prod_{1\le i\le N-1}(W_t^\ell-g_t^\ell(y_i))^{-\frac{2}{3}}}{(y_{N+1}-y_N)^{\frac{1}{2}}\times\prod_{1\le i\le N-1}(y_N-y_i)^{-\frac{2}{3}}}\times\frac{\LR_N(g_t^\ell(y_1),\ldots, g_t^\ell(y_{N-1}), W_t^\ell; g_t^\ell(y_{N+1}))}{\LR_N(y_1,\ldots,y_N;y_{N+1})}.
\end{align*}
Then, we have that $\{M_t\}_{t\ge 0}$ is a local martingale for $\ell$. For $\eps>0$ and $K>0$, define $\tau_\eps$ to be the hitting time of $\ell$ at the union of $\eps$-neighbourhood of $(y_{N+1},+\infty)$ and $\partial B(y_N,\frac{1}{\eps})$, define $L_K$ to be the first time that $M_t\ge K$. Then,  the law of $\ell$ weighted by $\left\{M_{t\wedge\tau_\eps\wedge L_K}\right\}_{t\ge 0}$ equals the law of $\gamma_N$ in Lemma~\ref{lem::conv_aux} stopped at corresponding stopping time.
\end{lemma}
\begin{proof}
The proof follows from the commutation relations for $\SLE$s~\cite{DubedatCommutationSLE}. 
We  first prove that  curves $(\gamma_1,\ldots,\gamma_N)\sim\mathcal Q$ satisfy the following commutation relation: Take any disjoint neighborhoods $U_1,\ldots, U_N$ such that $U_j$ contains $x_j$ on its boundary and $U_j\cap\left(\{x_1,\ldots,x_{j-1},x_{j+1},\ldots, x_{N}\}\cup [x_{N+1}x_{N+2}]\right)=\emptyset$ for $1\le j\le N$. Denote by $T_j$ the hitting time of $\gamma_j$ at $\overline{\partial U_j\cap\Omega}$. Denote by $\phi_T$ the conformal map from $\Omega_T:=\Omega\setminus\cup_{1\le i\le N}\gamma_i[0,T_i]$ onto $\HH$ such that $\phi_T(x_{N+2})=\infty$ and $\phi_T(\gamma_1(T_1))<\ldots<\phi_T(\gamma_N(T_N))<\phi_T(x_{N+1})$. Denote by $\tau_j$ the hitting time of $\gamma_j$ at $\cup_{i\neq j}\gamma_i[0,T_i]\cup (x_{N+1}x_{N+2})$. Then, the driving function of $\phi_T(\gamma_j[T_j,\tau_j))$ satisfies SDE~\eqref{eqn::local_driving} if we  replace $(\phi(x_1),\ldots,\phi(x_{N+1}))$ by $(\phi_T(\gamma_1(T_1)),\ldots,\phi_T(x_{N+1}))$.

Choose stopping times $T_j^\delta$ for $\gamma_j^{\delta_n}$ such that $T_j^\delta$ converges to $T_j$ almost surely under $\mathcal Q$. Then, we have that $\Omega_{T}^{\delta_n}:=\Omega_{\delta_n}\setminus\cup_{1\le i\le N}\gamma_i^{\delta_n}[0,T_i^{\delta_n}]$ converges to $\Omega_T$ in the Carath\'eodory sense almost surely. Choose conformal map $\phi^{\delta_n}_T$ from $\Omega_T^{\delta_n}$ onto $\HH$, such that $\phi^{\delta_n}_T(x^{\delta_n}_{N+2})=\infty$ and $\phi^{\delta_n}_T(\gamma^{\delta_n}_1(T^{\delta_n}_1))<\ldots<\phi^{\delta_n}_T(\gamma^{\delta_n}_N(T^{\delta_n}_N))<\phi^{\delta_n}_T(x^{\delta_n}_{N+1})$ and $\phi^{\delta_n}_T$ converges to $\phi_T$ locally uniformly. Denote by $\tau^{\delta_n}_j$ the hitting time of $\gamma^{\delta_n}_j$ at $\cup_{i\neq j}\gamma^{\delta_n}_i[0,T^{\delta_n}_i]\cup[x^{\delta_n}_{N+1}x^{\delta_n}_{N+2}]$.   
\begin{itemize}
\item
By~\cite[Theorem 3.1]{IzyurovObservableFree}, we have that the driving function of $\phi_T^{\delta_n}(\gamma_j^{\delta_n}[T_j^{\delta_n},\tau_j^{\delta_n}))$ converges the solution of SDE~\eqref{eqn::local_driving} in law if we  replace $(\phi(x_1),\ldots,\phi(x_{N+1}))$ by $(\phi_T(\gamma_1(T_1)),\ldots,\phi_T(x_{N+1}))$. 
\item
By the convergence of $\gamma_i^{\delta_n}$ for $1\le i\le N$, and the fact that the limit $\gamma_i$ is simple (due to Lemma~\ref{lem::conv_aux} and Lemma~\ref{lem::conv_aux2}), we have that the limit of the driving function of $\phi_T^{\delta_n}(\gamma_j^{\delta_n}[T_j^{\delta_n},\tau_j^{\delta_n}))$ equals the driving function of $\phi(\gamma_j[T_j,\tau_j))$ almost surely.
\end{itemize}
Combining these two facts together, we have that the driving function of $\phi(\gamma_j[T_j,\tau_j))$ satisfies the required SDE (See also~\cite[Remark 3.2]{IzyurovObservableFree}).
By~\cite[Theorem 7]{DubedatCommutationSLE}, there exists a constant $\mu\in\R$, such that on $\Xi_{N+1}$, we have
\begin{equation}\label{eqn::BPZ_aux}
\left(\frac{\kappa}{2}\partial_{ii}^2+\sum_{\substack{1\le j\le N+1\\j\neq i}}\frac{2}{y_j-y_i}\partial_j-\sum_{\substack{1\le j\le N\\j\neq i}}\frac{2h}{(y_j-y_i)^2}-\frac{2\mu}{(y_{N+1}-y_i)^2}\right)R=0
\end{equation}
By definition of $\LR_N$, we have 
\[\lim_{y_N\to y_{N+1}}(y_{N+1}-y_N)^2\partial^2_{NN}\LR_N(y_1,\ldots,y_N;y_{N+1})=\frac{3}{4}\LR_{N-1}(y_1,\ldots,y_{N-1};y_N)\]
and
\[\lim_{y_N\to y_{N+1}}(y_{N+1}-y_N)\partial_{N+1}\LR_N(y_1,\ldots,y_N;y_{N+1})=-\frac{1}{2}\LR_{N-1}(y_1,\ldots,y_{N-1};y_N).\]
By~\cite[Remark 2.5]{IzyurovObservableFree}, we have that $\LR_{N-1}(y_1,\ldots,y_{N-1};y_N)\neq 0$. Plugging into~\eqref{eqn::BPZ_aux}, we obtain $\mu=\frac{1}{16}$. This proves~\eqref{eqn::BPZ}.

By I\'to's formula, we can conclude that $\{M_t\}_{t\ge 0}$ is a local martingale for $\ell$. The last conclusion is due to the Girsanov's theorem. This completes the proof.
\end{proof}
\begin{lemma}\label{lem::bound_control}
For $K>0$, define
\[\Xi_{N+1,K}:=\left\{(y_1,\ldots,y_{N+1})\in\Xi_{N+1}: |y_i|\le K\text{ for }1\le i\le N+1\text{ and }|y_{i}-y_{i-1}|\ge\frac{1}{K}\text{ for }2\le i\le N\right\}.\]
Then, we have the following properties.
\begin{itemize}
\item
We have that $\LR_N>0$ on $\Xi_{N+1}$.
\item
 There exists a constant $C=C(K)>0$ such that
\[\sup_{(y_1,\ldots,y_{N+1})\in\Xi_{N+1,K}}\frac{\mathcal Z_N(y_1,\ldots,y_N;y_{N+1})}{\prod_{1\le i<j\le N}(y_j-y_i)^{-\frac{2}{3}}\prod_{1\le i\le N}(y_{N+1}-y_i)^{\frac{1}{2}}\times\LR_N(y_1,\ldots,y_N;y_{N+1})}\le C(K).\]
\end{itemize}
\end{lemma}
\begin{proof}
For the first item, we can prove by induction. Suppose it holds when $N\le n-1$, when $N=n$, we have
\[\lim_{n\to\infty}(y_{n}-y_{n-1})^{\frac{1}{2}}\LR_n(y_1,\ldots,y_{n-1};y_{n})=\LR_{n-1}( y_1,\ldots,\hat y_{n-2};\hat y_{n-1})>0.\]
By~\cite[Remark 2.5]{IzyurovObservableFree}, we have that $\LR_n$ is non-zero on $\Xi_{N+1}$. This implies that $\LR_n$ is positive on $\Xi_{N+1}$ and completes the proof of the first item.

For the second item, note that $\prod_{1\le i<j\le N}(y_j-y_i)^{-\frac{2}{3}}\prod_{1\le i\le N-1}(y_{N+1}-y_i)^{\frac{1}{2}}$ is uniformly bounded from above on $\Xi_{N+1,K}$. Similar to~\eqref{eqn::bound_U_1}, we have that  $\mathcal Z_N$ is uniformly bounded from above on $\Xi_{N+1,K}$.
Suppose $\{(y^n_1,\ldots,y^n_{N+1})\}_{n\ge 1}$ is a sequence of points such that 
\[
\lim_{n\to\infty}(y_{N+1}-y_N)^{\frac{1}{2}}\LR_N(y^n_1,\ldots,y^n_N;y^n_{N+1})=\inf_{(y_1,\ldots,y_{N+1})\in\Xi_{N+1,K}}(y_{N+1}-y_N)^{\frac{1}{2}}\LR_N(y_1,\ldots,y_N;y_{N+1}).
\]
We may assume that $\lim_{n\to\infty}y_j^n=\hat y_j$ for $1\le j\le N+1$.
\begin{itemize}
\item
If $\hat y_N\neq \hat y_{N+1}$, we have
\[\lim_{n\to\infty}(y_{N+1}-y_N)^{\frac{1}{2}}\LR_N(y^n_1,\ldots,y^n_N;y^n_{N+1})=(\hat y_{N+1}-\hat y_N)^{\frac{1}{2}}\LR_N(\hat y_1,\ldots,\hat y_N;\hat y_{N+1}),\]
which is nonzero by~\cite[Remark 2.5]{IzyurovObservableFree}.
\item
If $\hat y_N=\hat y_{N+1}$, we have
\[\lim_{n\to\infty}(y_{N+1}-y_N)^{\frac{1}{2}}\LR_N(y^n_1,\ldots,y^n_N;y^n_{N+1})=\LR_{N-1}(\hat y_1,\ldots,\hat y_{N-1};\hat y_{N}),\]
which is nonzero by~\cite[Remark 2.5]{IzyurovObservableFree}.
\end{itemize}
This completes the proof.
\end{proof}
Now, we come back to the proof of Theorem~\ref{thm::Ising_limit}. As in Lemma~\ref{lem::mart_gammaN}, denote by $y_j=\phi(x_j)$ for $1\le j\le N$. By Lemma~\ref{lem::curve_properties}, the second line and the third line in~\eqref{eqn::limt_prob} are equal to each other, which we denote by $F_N(y_1,\ldots,y_{N};y_{N+1})$.
\begin{proof}[Proof of Theorem~\ref{thm::Ising_limit}]
We will prove by induction. 

We first consider the case $N=1$. By Lemma~\ref{lem::conv_aux} and Lemma~\ref{lem::conv_aux1}, we have that $\gamma_1^\delta$ converges to $\SLE_3\left(-\frac{3}{2},-\frac{3}{2}\right)$. Due to the explicit form of $\mathcal Z_1,\mathcal W_1$ and $\LR_1$, the second line and the third line in~\eqref{eqn::limt_prob} equals $1$. Thus, Theorem~\ref{thm::Ising_limit} holds when $N=1$.

Next, suppose that Theorem~\ref{thm::Ising_limit} holds for $N\le m-1$. By tightness, It suffices to prove Theorem~\ref{thm::Ising_limit} when $N=m$ along a subsequence. By Lemma~\ref{lem::conv_aux2}, we can choose a subsequence, which we still denote by $\{\delta_n\}_{n\ge 1}$, such that $\one_{\{\gamma_N^{\delta_n}\text{ ends at }(x_{N+1}^\delta,x_{N+2}^\delta)\}}$ converges to $\one_{\{\tau<\sigma\}}$ almost surely under $\mathcal Q$. 

We first prove~\eqref{eqn::limt_prob} and derive the law of $\gamma_N$.
Denote by $\hat\Omega_{\delta_n}$ (resp. $\hat\Omega$) the connected component of $\Omega_{\delta}\setminus\gamma_N^{\delta_n}$ (resp. $\Omega\setminus\gamma_N$) which contains $x_1^{\delta_n}$ (resp. $x_1$). Then, we have that $\hat\Omega_{\delta_n}$ converges to $\hat\Omega$ in the close-Carath\'eodory sense. Denote by $\tau_{\delta_n}$ the hitting time of $\gamma_N^{\delta_n}$ at $(x_{N+1}^{\delta_n}x_{N+2}^{\delta_n})$. Suppose $f$ is a continuous and bounded function on curve space, by domain Markov property, we have
\[\E[\one_{A_{\delta_n}}f(\gamma_N^{\delta_n})]=\E\left[\E[A_{\delta_n}(\hat\Omega_{\delta_n};x_1^{\delta_n},\ldots,x_{N-1}^{\delta_n};\gamma_N^{\delta_n}(\tau_{\delta_n}),x_{N+2}^{\delta_n})]f(\gamma_N^{\delta_n})\one_{\{\gamma_N^{\delta_n}\text{ ends at }(x_{N+1}^\delta x_{N+2}^\delta)\}}\right]\]
 Denote by $(W_t:t\ge 0)$ the driving function of $\phi(\gamma_N)$ and by $(g_t:t\ge 0)$ the corresponding conformal maps. By induction hypothesis, we have that 
\begin{equation}\label{eqn::final_aux1}
\lim_{n\to\infty}\E[\one_{A_{\delta_n}}f(\gamma_N^{\delta_n})]=\mathcal Q\left[F_{N-1}(g_\tau(y_1),\ldots, g_\tau(y_{N-1}; W_\tau))f(\gamma_N)\one_{\{\tau<\sigma\}}\right].
\end{equation}
By Lemma~\ref{lem::cascade_eta} and Lemma~\ref{lem::mart_gammaN}, we have that $\{N_t:=F_N(g_t(y_1),\ldots, g_t(y_{N-1}),W_t; g_t(y_{N+1}))\}_{t\ge 0}$ is a local martingale for $\gamma_N$. Choose $K$ large enough. Recall the definition of $\Xi_{N+1,K}$ in Lemma~\ref{lem::bound_control}. Define $S_K$ the exiting time of $(g_t(y_1),\ldots, g_t(y_{N-1}),W_t; g_t(y_{N+1}))$ at $\Xi_{N+1,K}$. Denote by $\tau_\eps$ the hitting time of $\phi(\gamma_N)$ at the union of $\eps$-neighbourhood of $(y_{N+1},+\infty)$ and $\partial B(y_N,\frac{1}{\eps})$ and by $\sigma_\eps$ the hitting time of $\phi(\gamma_N)$ at $\eps$-neighbourhood of $\{y_1,\ldots,y_{N-1}\}$.
By Lemma~\ref{lem::bound_control}, there exists a constant $C(K)>0$ such that for every $t\ge 0$, we have 
\[N_{t\wedge\tau_\eps\wedge\sigma_\eps\wedge S_K}\le C(K).\]
Moreover, weighted by $\left\{\frac{N_{t\wedge\tau_\eps\wedge\sigma_\eps\wedge S_K}}{N_0}\right\}_{t\ge 0}$, the law of $\gamma_N[0,\tau_\eps\wedge\sigma_\eps\wedge S_K]$ equals the law of $\ell_N[0,\tau^{\ell_N}_\eps\wedge\sigma^{\ell_N}_\eps\wedge S^{\ell_N}_K]$ (See Theorem~\ref{thm::multiple_odd} for the definition of $\ell_N$), where we denote by $\tau^{\ell_N}_\eps,\sigma^{\ell_N}_\eps,S^{\ell_N}_K$ for $\ell_N$ similarly to $\tau_\eps, \sigma_\eps, S_K$. Thus, we have
\[
\mathcal Q[N_{\tau_\eps\wedge\sigma_\eps\wedge S_K}\one_{\{\sigma_\eps<\tau_\eps\wedge S_K\}}]=N_0\PP[\sigma^{\ell_N}_\eps<\tau^{\ell_N}_\eps\wedge S^{\ell_N}_K]
\]
In particular, since $\ell_N$ is a simple curve which hits $(y_{N+1},+\infty)$ before hitting $(-\infty, y_N)$, we have
\begin{equation}\label{eqn::mart_gammaN_aux1}
\lim_{\eps\to 0}\mathcal Q[N_{\tau_\eps\wedge\sigma_\eps\wedge S_K}\one_{\{\sigma_\eps<\tau_\eps\wedge S_K\}}]\le N_0\PP[\ell_N\text{ hits }\{y_1,\ldots, y_{N-1}\}]=0.
\end{equation}
On the event $\{\tau<\sigma\wedge S_K\}$, we have that 
\begin{align}\label{eqn::mart_gammaN_aux2}
&\lim_{\eps\to 0}N_{\tau_\eps}\notag\\
=&\frac{1}{B\left(\frac{2}{\kappa},\frac{2}{\kappa}\right)^{\left[\frac{N}{2}\right]}}\prod_{1\le i<j\le N-1}(g_\tau(y_j)-g_\tau(y_i))^{\frac{2}{3}}\prod_{1\le i\le N-1}(W_\tau-g_\tau(x_i))^{-\frac{1}{2}}\times\frac{\mathcal W_{N-1}(g_\tau(y_1),\ldots, g_\tau(y_{N-1});W_\tau)}{\LR_{N-1}(g_\tau(y_1),\ldots,g_\tau(y_{N-1});W-\tau)}\notag\\
=&F_{N-1}(g_\tau(y_1),\ldots, g_\tau(y_{N-1}; W_\tau)).
\end{align}
Denote the limit by $N_\tau$. Combining~\eqref{eqn::mart_gammaN_aux1} and~\eqref{eqn::mart_gammaN_aux2} together,  by letting $\eps\to 0$, we have 
\begin{equation}\label{eqn::mart_gammaN_aux3}
\mathcal Q[f(\gamma_N[0,\tau\wedge S_K])N_{\tau\wedge S_K}\one_{\{\tau\wedge S_K<\sigma\}}]=N_0\E\left[f(\ell_N[0,\tau^{\ell}_N\wedge S_K^{\ell_N}])\right].
\end{equation}
By letting $K\to \infty$, by dominated convergence theorem, we have
\begin{equation}\label{eqn::mart_gammaN_aux4}
\mathcal Q[f(\gamma_N[0,\tau])N_{\tau}\one_{\{\tau<\sigma\}}]=N_0\E\left[f(\ell_N[0,\tau^{\ell}_N])\right].
\end{equation}
By taking $f=1$ in~\eqref{eqn::final_aux1}, combining with~\eqref{eqn::mart_gammaN_aux4}, we have
\[\lim_{n\to \infty}\PP[A_{\delta_n}]=N_0.\]
This gives~\eqref{eqn::limt_prob}. Thus,~\eqref{eqn::final_aux1} and~\eqref{eqn::mart_gammaN_aux4} implies that
\begin{equation}\label{eqn::mart_gammaN_aux5}
\lim_{n\to\infty}\E[f(\gamma_N^{\delta_n})\cond A_{\delta_n}]=\E\left[f(\ell_N[0,\tau^{\ell}_N])\right].
\end{equation}
Thus, the conditional law of $\gamma_N^{\delta_n}$ given $A_{\delta_n}$ converges to $\ell_N$.

Next, by induction hypothesis, we have that the conditional law of $(\gamma_1^{\delta_n},\ldots,\gamma_{N-1}^{\delta_n})$ converges to multiple $N-1$-$\SLE_3\left(-\frac{3}{2},-\frac{3}{2}\right)$ on $X_{N-1}(\hat\Omega; x_1,\ldots,x_{N-1}; \gamma_N(\tau),x_{N+2})$. Combining with Theorem~\ref{thm::multiple_odd}, Theorem~\ref{thm::uniqueness_multiple} and~\eqref{eqn::weight_ell} and~\eqref{eqn::mart_gammaN_aux5}, we have that the random curves $(\gamma_1,\ldots,\gamma_N)$ is the multiple $N$-$\SLE_3\left(-\frac{3}{2},-\frac{3}{2}\right)$ on $X_{N}(\Omega; x_1,\ldots,x_{N}; x_{N+1},x_{N+2})$.

This completes the induction and hence completes the proof.
\end{proof}
